ThinkRL-Edit: Thinking in Reinforcement Learning for Reasoning-Centric Image Editing

Instruction-driven image editing with unified multimodal generative models has advanced rapidly, yet their underlying visual reasoning remains limited, leading to suboptimal performance on reasoning-centric edits. Reinforcement learning (RL) has been investigated for improving the quality of image editing, but it faces three key challenges: (1) limited reasoning exploration confined to denoising stochasticity, (2) biased reward fusion, and (3) unstable VLM-based instruction rewards. In this work, we propose ThinkRL-Edit, a reasoning-centric RL framework that decouples visual reasoning from image synthesis and expands reasoning exploration beyond denoising. To the end, we introduce Chain-of-Thought (CoT)-based reasoning sampling with planning and reflection stages prior to generation in online sampling, compelling the model to explore multiple semantic hypotheses and validate their plausibility before committing to a visual outcome. To avoid the failures of weighted aggregation, we propose an unbiased chain preference grouping strategy across multiple reward dimensions. Moreover, we replace interval-based VLM scores with a binary checklist, yielding more precise, lower-variance, and interpretable rewards for complex reasoning. Experiments show our method significantly outperforms prior work on reasoning-centric image editing, producing instruction-faithful, visually coherent, and semantically grounded edits.

==> sec/0_abstract.tex <==
\begin{abstract}
Instruction-driven image editing with unified multimodal generative models has advanced rapidly, yet their underlying visual reasoning remains limited, leading to suboptimal performance on reasoning-centric edits. Reinforcement learning (RL) has been investigated for improving the quality of image editing, but it faces three key challenges: (1) limited reasoning exploration confined to denoising stochasticity, (2) biased reward fusion, and (3) unstable VLM-based instruction rewards.
In this work, we propose \textbf{ThinkRL-Edit}, a reasoning-centric RL framework that decouples visual reasoning from image synthesis and expands reasoning exploration beyond denoising. To the end, we introduce Chain-of-Thought (CoT)–based reasoning sampling with planning and reflection stages prior to generation in online sampling, compelling the model to explore multiple semantic hypotheses and validate their plausibility before committing to a visual outcome. 
To avoid the failures of weighted aggregation, we propose an unbiased chain preference grouping strategy across multiple reward dimensions. Moreover, we replace interval-based VLM scores with a binary checklist, yielding more precise, lower-variance, and interpretable rewards for complex reasoning. Experiments show our method significantly outperforms prior work on reasoning-centric image editing, producing instruction-faithful, visually coherent, and semantically grounded edits.
\end{abstract}

% To avoid the pitfalls of weighted reward aggregation, we develop an unbiased chain preference optimization strategy that jointly ranks sampled reasoning chains across multiple reward dimensions. Moreover, we replace interval-based VLM scoring with a binary checklist evaluation to yield more precise, lower-variance, and interpretable rewards, especially for complex reasoning.
% Extensive experiments demonstrate that our approach substantially outperforms prior methods on reasoning-centric image editing, delivering edits that are instruction-faithful, visually coherent, and semantically grounded.

==> sec/approach.tex <==
\section{Approach}

%\subsection{Hello World}

==> sec/experiments.tex <==
\section{Experiments}

%\subsection{Hello World}


\section{Conclusion}

==> sec/introduction.tex <==
\section{Introduction}

%\subsection{Hello World}

==> sec/relatedwork.tex <==
\section{Related Work}

%\subsection{Hello World}
